Ensemble Methods for Personalized E-Commerce Search Challenge at CIKM Cup 2016

Personalized search has been a hot research topic for many years and has been widely used in e-commerce. This paper describes our solution to tackle the challenge of personalized e-commerce search at CIKM Cup 2016. The goal of this competition is to predict search relevance and re-rank the result items in SERP according to the personalized search, browsing and purchasing preferences. Based on a detailed analysis of the provided data, we extract three different types of features, i.e., statistic features, query-item features and session features. Different models are used on these features, including logistic regression, gradient boosted decision trees, rank svm and a novel deep match model. With the blending of multiple models, a stacking ensemble model is built to integrate the output of individual models and produce a more accurate prediction result. Based on these efforts, our solution won the champion of the competition on all the evaluation metrics.

==> sig-alternate-aux <==
\relax 
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces the flowchart of our solution.}}{\thepage }}
\newlabel{fig:flowchart}{{1}{\thepage }}
\citation{cockburn2003revisit}
\citation{crammer2001pranking}
\citation{shashua2002ranking}
\citation{chu2005new}
\citation{herbrich1999large}
\citation{freund2003efficient}
\citation{burges2005learning}
\citation{quoc2007learning}
\citation{cao2007learning}
\citation{burges2010ranknet}
\citation{dietterich2000ensemble}
\citation{ratsch2001soft}
\citation{friedman2001greedy}
\citation{wolpert1992stack}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces  Basic statistics of the provided dataset.}}{\thepage }}
\newlabel{tab:stat1}{{1}{\thepage }}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces  User statistics of the provided dataset.}}{\thepage }}
\newlabel{tab:stat2}{{2}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {2}Dataset Overview}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {3}Related Work}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Learning to rank}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}Ensemble learning}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {4}Feature Extraction}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}Statistic Features}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.1.1}global statistic features}{\thepage }}
\citation{robertson2009probabilistic}
\newlabel{equ:1}{{1}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.1.2}Time-based statistic features}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}Query-Item Features}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.2.1}Category-based token features}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.2.2}Cross token features}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3}Session features}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {5}Model Framework}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1}Model Selection}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces deep match model.}}{\thepage }}
\newlabel{fig:dmm}{{2}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces the framework of query full.}}{\thepage }}
\newlabel{fig:queryfull}{{3}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2}Ensemble Modeling}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.2.1}Query Full}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.2.2}Query Less}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces the framework of query less.}}{\thepage }}
\newlabel{fig:queryless}{{4}{\thepage }}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces  Validation results of different models in our solution.}}{\thepage }}
\newlabel{tab:1}{{3}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {6}Results}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {7}Conclusions}{\thepage }}
\bibstyle{abbrv}
\bibdata{sigproc}
\bibcite{burges2005learning}{1}
\bibcite{burges2010ranknet}{2}
\bibcite{cao2007learning}{3}
\bibcite{chu2005new}{4}
\bibcite{crammer2001pranking}{5}
\bibcite{dietterich2000ensemble}{6}
\bibcite{freund2003efficient}{7}
\bibcite{friedman2001greedy}{8}
\bibcite{herbrich1999large}{9}
\bibcite{quoc2007learning}{10}
\bibcite{ratsch2001soft}{11}
\bibcite{robertson2009probabilistic}{12}
\bibcite{shashua2002ranking}{13}
\bibcite{wolpert1992stack}{14}
\@writefile{toc}{\contentsline {section}{\numberline {8}Acknowledgments}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {9}References}{\thepage }}

